A Note on the Gains from Trade of the Random-Offerer Mechanism

We study the classic bilateral trade setting. Myerson and Satterthwaite show that there is no Bayesian incentive compatible and budget-balanced mechanism that obtains the gains from trade of the first-best mechanism. Consider the random-offerer mechanism: with probability $\frac{1}{2}$ run the \emph{seller-offering} mechanism, in which the seller offers the buyer a take-it-or-leave-it price that maximizes the expected profit of the seller, and with probability $\frac{1}{2}$ run the \emph{buyer-offering} mechanism. Very recently, Deng, Mao, Sivan, and Wang showed that the gains from trade of the random-offerer mechanism is at least a constant factor of $\frac 1 {8.23}\approx 0.121$ of the gains from trade of the first best mechanism. Perhaps a natural conjecture is that the gains-from-trade of the random-offerer mechanism, which is known to be at least half of the gains-from-trade of the second-best mechanism, is also at least half of the gains-from-trade of the first-best mechanism. However, in this note we exhibit distributions such as the gains-from trade of the random-offerer mechanism is smaller than a $0.495$-fraction of the gains-from-trade of the first-best mechanism.

==> model.tex <==
\section{The Setting}

We consider bilateral trade settings with a seller that holds an indivisible item and a buyer that is interested in buying that item. 
The private value of the seller for keeping the item is $s\geq 0$ (and zero if he gives the item) and the private value of the buyer if he obtains the item is $b\geq 0$ (and zero otherwise). 
We assume that $s$ is independently drawn from a distribution $\FS$ and $b$ is independently drawn from $\FB$. $\FS$ and $\FB$ are known to both players. 

For a setting $(\FS,\FB)$, the \emph{optimal gains from trade (GFT)} is  
$OPT_{\FS, \FB}=E_{s\sim \FS, b\sim \FB}(b-s)_+=E_{s\sim \FS, b\sim \FB}[\max \{b-s,0\}]$.
In the \emph{seller-offering} mechanism, a seller with value $s$ that faces a buyer distribution $\FB$ posts a price $p = p_s(\FB)$ that maximizes his utility $\Pr_{b\sim \FB} [b\geq p]\cdot (p-s)$ (we will see that our assumptions on the distribution guarantee the existence of such price). Trade happens at price $p$ if and only if the buyer value $b$ is at least $p$ and the seller's value is at most $p$. When there are several prices that maximize this expression, we assume that the seller offers the highest price that maximizes this expression. If no price gives positive utility, i.e., if $\Pr[b>s]=0$, We will set the price to $\infty$ and sell never occurs in this case.

In the \emph{buyer-offering} mechanism, a buyer with value $b$ that faces a seller distribution $\FS$ posts a price $p= p_b(\FS)$ that maximizes $\Pr_{s\sim \FS} [s\leq p]\cdot (b-p)$ (again, our assumptions about the distributions guarantee that such $p$ exists). If there are several values of $p$ that maximize this expression, we choose the lowest one. Trade happens at price $p$ if and only if the seller value $s$ is at most $p$.  If no price $p$ gives positive utility, we let the price be $0$. Finally, let the \emph{random-offerer} mechanism be the mechanism that  with probability half runs the buyer-offering mechanism and with probability half runs the seller-offering mechanism. Observe that each of the mechanisms above is Bayesian incentive compatible, ex-post IR and strongly budget balanced.
%Note that the expected GFT of the random-offerer mechanism is at most the GFT of the higher GFT of the two mechanisms. 

%Observe that the buyer-offering mechanism can be implemented as a direct revelation mechanism in which the buyer reports his value and the mechanism posts a price that equals to the buyer offer (maximizing the buyer's utility). Such a mechanism (with zero payment if there is no trade) is BIC, ex-post IR and strongly budget balanced. Similar claim holds for the seller-offering mechanism. 

%By the Myerson-Satterthwaite \cite{} impossibility result,  for non-trivial instances 
%there does not exist a Bayesian Incentive Compatible (BIC), interim individually rational and weakly budget-balanced mechanism with GFT that is equal to the optimal GFT. 
%We ask if there exists and truthful mechanism (that is individually rational and budget-balanced) that \emph{approximates} the optimal GFT. 
%We show that the random-offerer mechanism is  a Bayesian Incentive Compatible (BIC), ex-post individually rational and strongly budget-balanced mechanism that has expected GFT that is at least half the optimal gains from trade. As the GFT of the random-offerer is the average of the GFT of the seller-offering and buyer-offering mechanisms,  
%we conclude that either the buyer-offering mechanism or the seller-offering mechanism is a Bayesian Incentive Compatible (BIC), ex-post individually rational and strongly budget-balanced mechanism that  has expected GFT that is at least half the optimal expected GFT.
%\mbcomment{we probably need to define all the terms: BIC, IR, BB etc.} 

For any two bounded distributions $\FS$ and $\FB$ for which the seller-offering and buyer-offering mechanisms are both well defined, we denote the expected gains from trade (GFT) of the seller-offering mechanism by $SO_{\FS, \FB}$ and the expected GFT of the buyer-offering mechanism by $BO_{\FS, \FB}$. 
Note that the expected GFT of the random-offerer mechanism is  $(BO_{\FS,\FB}+SO_{\FS,\FB})/2$. 
We sometimes omit the subscripts $\FS, \FB$ when the distributions are clear from the context.

%The \emph{approximation ratio} of the random-offerer mechanism is:
%\begin{equation*}
%R({\FS,\FB})=
%\frac {OPT_{\FS,\FB}} {\frac{1}{2}(BO_{\FS,\FB}+SO_{\FS,\FB})} 
% = 2\cdot \frac {OPT_{\FS,\FB}} {BO_{\FS,\FB}+SO_{\FS,\FB}}
%\end{equation*}
%As the case that $OPT_{\FS,\FB}=0$ is trivial (any mechanism is optimal), throughout the paper we only consider non-trivial settings, ones in which  $OPT_{\FS,\FB}>0$. If the denominator is $0$, we define the ratio to be $\infty$. 

